BPO: Towards Balanced Preference Optimization between Knowledge Breadth and Depth in Alignment

Reinforcement Learning with Human Feedback (RLHF) is the key to the success of large language models (LLMs) in recent years. In this work, we first introduce the concepts of knowledge breadth and knowledge depth, which measure the comprehensiveness and depth of an LLM or knowledge source respectively. We reveal that the imbalance in the number of prompts and responses can lead to a potential disparity in breadth and depth learning within alignment tuning datasets by showing that even a simple uniform method for balancing the number of instructions and responses can lead to significant improvements. Building on this, we further propose Balanced Preference Optimization (BPO), designed to dynamically augment the knowledge depth of each sample. BPO is motivated by the observation that the usefulness of knowledge varies across samples, necessitating tailored learning of knowledge depth. To achieve this, we introduce gradient-based clustering, estimating the knowledge informativeness and usefulness of each augmented sample based on the model's optimization direction. Our experimental results across various benchmarks demonstrate that BPO outperforms other baseline methods in alignment tuning while maintaining training efficiency. Furthermore, we conduct a detailed analysis of each component of BPO, providing guidelines for future research in preference data optimization.

==> latex/experimental_results-org.tex <==

In this section, we analyze our main experimental results. 
% We first examine the impact of selecting fewer prompts using embedding-based clustering (\textit{Less Prompt}) and uniformly expanding these prompts with additional response pairs to match the original dataset size (\textit{Less Prompt + More Response}). 

% Then, we analyze the results of fine-tuning using the informative response pairs selected by gradient-based clustering from the constructed pairs. 
% Notably, we consistently perform SFT on the seed data before perform DPO with different selected data.

% \paragraph{Less Prompts and More Responses} 
% In Table~\ref{tab: less prompt}, we demonstrate that using embedding-based clustering to select only 5\% to 10\% of the representative prompts for alignment can achieve performance comparable to, and even surpassing, alignment on the full dataset while significantly reducing computational resource requirements.
% % This indicates that a representative narrower learning space can efficiently align the model. 
% Furthermore, deepening the learning space by constructing diverse responses for these selected prompts leads to further improvements in model performance
% These results highlight that a narrower and deeper learning space enables more efficient alignment of the model.

\paragraph{Performance of BPO}
Our alignment results using the informative response pairs selected through gradient-based clustering are presented in Table~\ref{tab: main exp}. 
Our method generally outperforms both KBS as described Section~\ref{prompts selection} and uniformly increasing the number of responses (\textit{10\% sampled prompts w/ UI}) across models of different sizes. 
Additionally, we compare our method with random selection of 10\% of the uniformly increased pairs (\textit{10\% sampled prompts w/ random select 10\% UI}) and the original full dataset (\textit{Fullset}). 
The results show that our method consistently achieves superior performance.
This indicates that our hierarchical clustering-based framework effectively refines the learning space, allocates dynamic learning depth for various prompts, and leads to better results.

% In Table \ref{tab: ours safe} and Table \ref{tab: ours HH}, we first reduce the dataset by selecting 10\% of the prompts (referred to as "Less Prompt")
% The second step compares DPO performance on the full dataset vs selected data using three approaches for response pair selection after preliminary SFT on the same seed data: 
% (1) no further selection, 
% (2) random selection of 10\% of the constructed response pairs, and
% (3) gradient-based clustering to select 10\% of the constructed response pairs (ours). 
% All experiments are conducted using Llama-3-8B and Llama-2-13B models.
